Look, Zoom, Understand: The Robotic Eyeball for Embodied Perception

In embodied AI, visual perception should be active rather than passive: the system must decide where to look and at what scale to sense to acquire maximally informative data under pixel and spatial budget constraints. Existing vision models coupled with fixed RGB-D cameras fundamentally fail to reconcile wide-area coverage with fine-grained detail acquisition, severely limiting their efficacy in open-world robotic applications. We study the task of language-guided active visual perception: given a single RGB image and a natural language instruction, the agent must output pan, tilt, and zoom adjustments of a real PTZ (pan-tilt-zoom) camera to acquire the most informative view for the specified task. We propose EyeVLA, a unified framework that addresses this task by integrating visual perception, language understanding, and physical camera control within a single autoregressive vision-language-action model. EyeVLA introduces a semantically rich and efficient hierarchical action encoding that compactly tokenizes continuous camera adjustments and embeds them into the VLM vocabulary for joint multimodal reasoning. Through a data-efficient pipeline comprising pseudo-label generation, iterative IoU-controlled data refinement, and reinforcement learning with Group Relative Policy Optimization (GRPO), we transfer the open-world understanding of a pre-trained VLM to an embodied active perception policy using only 500 real-world samples. Evaluations on 50 diverse real-world scenes across five independent evaluation runs demonstrate that EyeVLA achieves an average task completion rate of 96%. Our work establishes a new paradigm for instruction-driven active visual information acquisition in multimodal embodied systems.

==> sec/limitations.tex <==


% \noindent\textbf{Limitation.} Although this method achieves impressive performance in open-world active visual perception tasks, it is still constrained by the high computational demands of VLMs and the limitations of the camera's hardware, which affecting its applicability in real-time scenarios. These limitations can be alleviated by using lightweight VLMs and advancements in hardware technology. 

% Furthermore, although we use a zoom-capable camera to perform "zoom in" operations, enabling finer-grained perception over a broader area within spatial constraints, hardware limitations still hinder the exploration of more comprehensive active perception strategies, such as "zoom out" after zooming in to capture global contextual information from other regions. Our future work may extend this system to support multi-step visual perception across multiple instruction rounds, thereby enabling more flexible and adaptive active visual perception capabilities.

\noindent\textbf{Limitation.}
Although this method achieves strong performance in open-world active visual perception tasks, it remains constrained by the high computational demands of VLMs and the physical limitations of camera hardware, which affect its applicability in real-time scenarios. These limitations may be mitigated through the use of lightweight VLM architectures and continued advancements in edge computing and sensor hardware.

Furthermore, while our evaluation includes 50 held-out real-world scenes with novel object instances and environments not observed during training, this scale does not yet match the large-scale open-world evaluation commonly seen in static vision benchmarks. Nevertheless, following embodied AI evaluation conventions, this setup represents a rigorous real-world assessment given the substantial cost of physical data collection and annotation, with each scene requiring approximately 30 minutes of manual labeling.

% In addition, although our system leverages a zoom-capable camera to perform active "zoom-in" operations for fine-grained perception, hardware constraints currently limit more comprehensive perception strategies. For example, dynamically performing multi-step zoom-in and zoom-out exploration to recover global context after local inspection remains challenging. Future work will extend the system to support multi-step, instruction-conditioned visual exploration across multiple perception rounds, enabling more flexible, adaptive, and globally consistent active perception.



